Avoiding Burst-like Error Patterns in Windowed Decoding of Spatially Coupled LDPC Codes

In this work, we analyze efficient window shift schemes for windowed decoding of spatially coupled low-density parity-check (SC-LDPC) codes, which is known to yield close-tooptimal decoding results when compared to full belief propagation (BP) decoding. However, a drawback of windowed decoding is that either a significant amount of window updates are required leading to unnecessary high decoding complexity or the decoder suffers from sporadic burst-like error patterns, causing a decoder stall. To tackle this effect and, thus, to reduce the average decoding complexity, the basic idea is to enable adaptive window shifts based on a bit error rate (BER) prediction, which reduces the amount of unnecessary updates. As the decoder stall does not occur in analytical investigations such as the density evolution (DE), we examine different schemes on a fixed test-set and exhaustive monte-carlo simulations based on our graphic processing unit (GPU) simulation framework. As a result, we can reduce the average decoding complexity of the naive windowed decoder while improving the BER performance when compared to a non-adaptive windowed decoding scheme. Furthermore, we show that a foresightful stall prediction does not significantly outperform a retrospective stall detection which is much easier to implement in practice.

==> acronyms.tex <==
\begin{acronym}
 \acro{ADC}{analog-to-digital converter}
 \acro{AGC}{automatic gain control}
 \acro{ASIC}{application-specific integrated circuit}
 \acro{AWGN}{additive white Gaussian noise}
 \acro{BER}{bit error rate}
 \acro{BICM}{bit interleaved coded modulation}
 \acro{BLER}{block error rate}
 \acro{CFO}{carrier frequency offset}
 \acro{DL}{deep learning}
 \acro{DQPSK}{differential quadrature phase-shift keying}
 \acro{ECC}{error correcting code}
 \acro{FPGA}{field programmable gate array}
 \acro{GNR}{GNU Radio}
 \acro{GPU}{graphic processing unit}
 \acro{ISI}{inter-symbol interference}
 \acro{LOS}{line-of-sight}
 \acro{MIMO}{multiple-input multiple-output}
 \acro{ML}{machine learning}
 \acro{MLP}{multilayer perceptron}
 \acro{MSE}{mean squared error}
 \acro{NN}{neural network}
 \acro{PLL}{phase-locked loop}
 \acro{ppm}{parts per million}
 \acro{PSK}{phase-shif keying}
 \acro{PFB}{polyphase filterbank}
 \acro{QAM}{quadrature amplitude modulation}
 \acro{ReLU}{rectified linear unit}
 \acro{RNN}{recurrent neural network}
 \acro{RRC}{root-raised cosine}
 \acro{RTN}{radio transformer network}
 \acro{SDR}{software-defined radio}
 \acro{SFO}{sampling frequency offset}
 \acro{SGD}{stochastic gradient descent}
 \acro{SNR}{signal-to-noise ratio}	
 \acro{TDL}{tapped delay line}
 \acro{OFDM}{orthogonal frequency division multiplex}
 \acro{IFFT}{inverse fast Fourier transform}
 \acro{FFT}{fast Fourier transform}
 \acro{IFT}{inverse Fourier transform}
 \acro{FT}{Fourier transform}
 \acro{IDFT}{inverse discrete Fourier-transform}
 \acro{DFT}{discrete Fourier-transform}
 \acro{CP}{cyclic prefix}
 \acro{MMSE}{minimum mean squared error}
 \acro{QPSK}{quadrature phase-shift keying}
 \acro{BP}{belief propagation}
 \acro{SC}{spatial coupling}
 \acro{LDPC}{low-density parity-check}
 \acro{SC-LDPC}{spatially coupled low-density parity-check}
 \acro{DE}{density evolution}
 \acro{MAP}{maximum a posteriori}
 \acro{VN}{variable node}
 \acro{CN}{check node}
 \acro{LLR}{log likelihood ratio}
\end{acronym}

==> corporateColours.tex <==
\definecolor{mittelblau}{RGB}{0, 126, 198}
\definecolor{violettblau}{cmyk}{0.9, 0.6, 0, 0}
\definecolor{rot}{RGB}{238, 28 35}
\definecolor{apfelgruen}{RGB}{140, 198, 62}
\definecolor{gelb}{RGB}{1, 221, 0}
\definecolor{orange}{RGB}{244, 111, 33}
\definecolor{pink}{RGB}{237, 0, 140}
\definecolor{lila}{RGB}{128, 10, 145}
\definecolor{hellgrau}{RGB}{224, 224, 224}
\definecolor{mittelgrau}{RGB}{128, 128, 128}
\definecolor{dunkelgrau}{RGB}{80,80,80}
\definecolor{anthrazit}{RGB}{19, 31, 31}


